GARCIA: Powering Representations of Long-tail Query with Multi-granularity Contrastive Learning

Recently, the growth of service platforms brings great convenience to both users and merchants, where the service search engine plays a vital role in improving the user experience by quickly obtaining desirable results via textual queries. Unfortunately, users' uncontrollable search customs usually bring vast amounts of long-tail queries, which severely threaten the capability of search models. Inspired by recently emerging graph neural networks (GNNs) and contrastive learning (CL), several efforts have been made in alleviating the long-tail issue and achieve considerable performance. Nevertheless, they still face a few major weaknesses. Most importantly, they do not explicitly utilize the contextual structure between heads and tails for effective knowledge transfer, and intention-level information is commonly ignored for more generalized representations. To this end, we develop a novel framework GARCIA, which exploits the graph based knowledge transfer and intention based representation generalization in a contrastive setting. In particular, we employ an adaptive encoder to produce informative representations for queries and services, as well as hierarchical structure aware representations of intentions. To fully understand tail queries and services, we equip GARCIA with a novel multi-granularity contrastive learning module, which powers representations through knowledge transfer, structure enhancement and intention generalization. Subsequently, the complete GARCIA is well trained in a pre-training&fine-tuning manner. At last, we conduct extensive experiments on both offline and online environments, which demonstrates the superior capability of GARCIA in improving tail queries and overall performance in service search scenarios.

==> tab/dataset_amazon.tex <==
\begin{table}
    % \scriptsize
	\caption{The statistics of three offline datasets.}
	\label{tab:dataset_amazon}
\centering
\setlength{\tabcolsep}{1.6mm}{
	\begin{tabular}{c|c|c|c|c}
		\toprule
        \multicolumn{2}{c|}{} & {Software} & {Video\_game} & {Musical\_Instruments} \\
        \midrule
         \multirow{2}{*}{\# Queries} &{Head} & {10.95\%} & {3.62\%} & {3.63\%} \\
        %\hline{2-5}
        {} &{Tail} & {89.05\%} & {96.38\%} & {96.37\%} \\
        \midrule
        \multirow{2}{*}{\# Search PV} &{Head} & {23.44\%} & {17.31\%} & {13.57\%} \\
        %\hline{2-5}
        {} &{Tail} & {76.56\%} & {82.69\%} & {86.43\%} \\
        % \midrule
        % \multicolumn{2}{c|}{\# Items}& {} & {} & {} \\
        % \midrule
        % \multicolumn{2}{c|}{\# Intentions}& {} & {} & {} \\
        % \midrule
        \midrule 
        \multicolumn{2}{c|}{\# Train} & {$8.96 \times 10^3$} & {$3.48 \times 10^5$} & {$1.62 \times 10^5$} \\
        \midrule
        % \multicolumn{2}{c|}{\# Validation} & \multicolumn{3}{c}{1,000,000} \\
        % \multicolumn{2}{c|}{\# Validation} & \multicolumn{3}{c}{$1 \times 10^6$} \\
        % \midrule 161974
        % \multicolumn{2}{c|}{\# Test} & \multicolumn{3}{c}{1,000,000} \\
        \multicolumn{2}{c|}{\# Test} & {$3.84 \times 10^3$} & {$1.49 \times 10^5$} & {$6.94 \times 10^4$} \\
        % \midrule
        % \midrule
        % \multicolumn{2}{c|}{\# Nodes} & {} & {} & {} \\
        % \midrule
        % \multicolumn{2}{c|}{\# Edges} & {} & {} & {} \\
        % \midrule
        % \multicolumn{2}{c|}{\# Attributes}& {} & {} & {} \\
         
		\bottomrule
	\end{tabular}}
\end{table}



==> tab/dataset_graph_amazon.tex <==
\begin{table}
    % \scriptsize
	\caption{The statistics of search service graph and Category tree.}
	\label{tab:dataset_graph_amazon}
\centering
\setlength{\tabcolsep}{3.5mm}{
	\begin{tabular}{c|c|c|c}
		\toprule
        {} & {Head } & {Tail} &  \multirow{2}{*}{Category tree}\\
		{} & \multicolumn{2}{c|}{Software} & {} \\

        \midrule
        % {\# Nodes} & {1,753,368} & {2,401,692} & {3,254} \\
        {\# Nodes} & {$8.61 \times 10^2$} & {$2.42 \times 10^3$} & {$- \times 10^3$} \\
        \midrule
        % {\# Edges} & {374,806} & {2,000,956} & {3,289} \\
        {\# Edges} & {$2.79 \times 10^3$} & {$9.10 \times 10^3$} & {$- \times 10^3$} \\
        % \midrule
        % {\# Attributes}& \multicolumn{2}{c|}{11} & {N.A.} \\
        \midrule
		{} & \multicolumn{2}{c|}{Video\_game} & {Category tree} \\
        % {} & {Head } & {Tail} &  {}\\
        \midrule
        % {\# Nodes} & {1,753,368} & {2,401,692} & {3,254} \\
        {\# Nodes} & {$1.65 \times 10^4$} & {$7.06 \times 10^4$} & {$- \times 10^3$} \\
        \midrule
        % {\# Edges} & {374,806} & {2,000,956} & {3,289} \\
        {\# Edges} & {$8.16 \times 10^4$} & {$3.92 \times 10^5$} & {$- \times 10^3$} \\
        % \midrule
        % {\# Attributes}& \multicolumn{2}{c|}{11} & {N.A.} \\
        \midrule
		{} & \multicolumn{2}{c|}{Musical\_Instruments} & {Category tree} \\
        % {} & {Head } & {Tail} &  {}\\
        \midrule
        % {\# Nodes} & {1,753,368} & {2,401,692} & {3,254} \\
        {\# Nodes} & {$8.79 \times 10^3$} & {$3.71 \times 10^4$} & {$- \times 10^3$} \\
        \midrule
        % {\# Edges} & {374,806} & {2,000,956} & {3,289} \\
        {\# Edges} & {$2.95 \times 10^4$} & {$1.90 \times 10^5$} & {$- \times 10^3$} \\
        % \midrule
        % {\# Attributes}& \multicolumn{2}{c|}{11} & {N.A.} \\
         
		\bottomrule
	\end{tabular}}
\end{table}



==> tab/eff_exp_table_3.tex <==
 %\usepackage[normalem]{ulem}
 %\useunder{\uline}{\ul}{}
% \begin{table*}
%     % \scriptsize
% 	\caption{Performance comparison \wrt AUC with baselines on three datasets.}
% 	\label{tab:baseline}
% \centering
% \setlength{\tabcolsep}{4.5mm}{
% 	\begin{tabular}{c|c|c|c|c|c|c|c}
% 		\toprule
%         {} & {} & {Wide\&Deep} & {LightGCN} & {KGAT} & {SGL} & {SimSGL} & {{\model} (\emph{v.s.} best)} \\
% 		\midrule
% 		{} & {Head} & {0.8676} & {0.9199} & {0.9310} & {0.9291} &   {0.9333} & \textbf{0.9361 (+0.65\%)} \\
% 		{Sep. A} & {Tail} & {0.7581} & {0.8205} & {0.8169} & {0.8024} & {0.8142} & {\textbf{0.8285 (+2.50\%)}}\\
% 		{} & {Overall} & {0.8629} & {0.9156} & {0.9264} & {0.9241} & {{0.9286}} & \textbf{0.9320 (+0.78\%)}\\
% 		\midrule
% 	    {} & {Head}  & {0.8627} & {0.9084} & {0.9290} & {{0.9312}} & {0.9140} & \textbf{0.9332 (+0.46\%)}\\
% 		{Sep. B} & {Tail} & {0.7484} & {0.8172} & {0.8245} & {0.8175} & {0.7781} & {\textbf{0.8374 (+3.96\%)}}\\
% 		{} & {Overall} & {0.8518} & {0.9034} & {{0.9239}} & {0.9258} & {0.9073} & {\textbf{0.9284 (+0.61\%)}} \\
% 		\midrule
% 	     {} & {Head} & {0.8618} & {0.9060} & {0.9239} & {0.9227} & {0.9202} & {\textbf{0.9248 (+0.22\%)}}\\
% 		{Sep. C} & {Tail} & {0.7468} & {0.8171} & {0.8191} & {0.8064} & {0.8088} & {\textbf{0.8310 (+3.73\%)}}\\
% 		{} & {Overall} & {0.8533} & {0.9012} & {0.9189} & {0.9173} & {0.9149} & {\textbf{0.9203 (+0.32\%)}}\\
% 		\midrule
% 	     {} & {Head} & {} & {} & {} & {} & {} & {}\\
% 		{Amazon} & {Tail} & {} & {} & {} & {} & {} & {}\\
% 		{} & {Overall} & {} & {} & {} & {} & {} & {}\\
% 		\bottomrule
% 	\end{tabular}}
% \end{table*}


\begin{table*}
    % \scriptsize
	\caption{\textcolor{red}{Performance comparison \wrt AUC with baselines on three datasets.}}
	\label{tab:baseline2}
\centering
\setlength{\tabcolsep}{3mm}{
	\begin{tabular}{c|c|c|c|c|c|c|c|c|c}
		\toprule
        {}  & \multicolumn{3}{c|}{Amazon-Software} & \multicolumn{3}{c|}{Amazon-Video game} & \multicolumn{3}{c}{Amazon-Music} \\
        \midrule
        {} & {Head} & {Tail} & {Overall} & {Head} & {Tail} & {Overall} & {Head} & {Tail} & {Overall}  \\
        \midrule
        {Wide\&Deep} & {0.7513} & {0.7483} & {0.7483} & {0.6443} & {0.5564} & {0.5712} & {0.6074} & {0.5841} & {0.5972} \\
        {LightGCN} & {0.8481} & {0.8202} & {0.8263} & {0.8025} & {0.7475} & {0.7562} & {0.6585} & {0.6635} & {0.6610}\\
        {KGAT} & {0.8190} & {0.8342} & {0.8280} & {0.7931} & {0.7605} & {0.7637} & {0.6750} & {0.6813} & {0.6746}\\
        {SGL} & {0.8182} & {0.8099} & {0.7989} & {0.7878} & {0.7610} & {0.7654} & {0.6512} & {0.6712} & {0.6515}\\
        {SimSGL} & {0.8571} & {0.8144} & {0.8248} & \textbf{0.8075} & {0.7671} & {0.7746} & {0.6512} & {0.6712} & {0.6515}\\
        \midrule
        {{\model}} & {\textbf{0.8605}} & {\textbf{0.8399}} & {\textbf{0.8436}} & {0.8060} & {\textbf{0.7713}} & {\textbf{0.7763}} & \textbf{0.6758} & {\textbf{0.7094}} & {\textbf{0.6906}} \\
        {(\emph{v.s.} best)} & {\textbf{+0.95\%}} & {\textbf{+1.71\%}} & {\textbf{+4.76\%}} & {-0.48\%} & {\textbf{+1.57\%}} & {\textbf{+0.62\%}} & \textbf{+0.45\%} & {\textbf{+15.50\%}} & {\textbf{+9.16\%}} \\
		\bottomrule
	\end{tabular}}
\end{table*}



==> tab/para_table.tex <==
\begin{table}
    % \scriptsize
	\caption{Parameter values used in {\model}.}
	\label{tab:para}
\centering
\setlength{\tabcolsep}{3.5mm}{
	\begin{tabular}{c|c|c|c|c|c}
	    \toprule
	    {} & {$H$} & {$L$} & {$\alpha$} & {$\beta$} & {$\tau$} \\
	    \midrule
	    {Sep. A} & {5} & {2} & {0.1} & {0.01} & {0.1} \\
	    {Sep. B} & {5} & {2} & {0.1} & {0.01} & {0.1}\\
        {Sep. C} & {2} & {2} & {0.1} & {0.01} & {0.1}\\
        \bottomrule
	\end{tabular}}
\end{table}


